The Impact of Revealing Large Language Model Stochasticity on Trust, Reliability, and Anthropomorphization

Interfaces for interacting with large language models (LLMs) are often designed to mimic human conversations, typically presenting a single response to user queries. This design choice can obscure the probabilistic and predictive nature of these models, potentially fostering undue trust and over-anthropomorphization of the underlying model. In this paper, we investigate (i) the effect of displaying multiple responses simultaneously as a countermeasure to these issues, and (ii) how a cognitive support mechanism-highlighting structural and semantic similarities across responses-helps users deal with the increased cognitive load of that intervention. We conducted a within-subjects study in which participants inspected responses generated by an LLM under three conditions: one response, ten responses with cognitive support, and ten responses without cognitive support. Participants then answered questions about workload, trust and reliance, and anthropomorphization. We conclude by reporting the results of these studies and discussing future work and design opportunities for future LLM interfaces.

==> notes.tex <==
%Observations based on question.
Advice (work-life)
- Short response seemed less human like
- Response was general and did not include context of the prompt
- Responses assumed that the person worked too much and needed to step away from work, not that they needed suggestions on how to work more efficiently because the “life aspect” was more consuming
- Model does not have personal information to answer the question well
- Interesting note: participant assumed that prompts were kept privacy 
Fact based (jupiter-saturn)
- Short responses more terse, less free flowing
- Shorter answers seem more human like because the longer responses seem to be “searching” for the answer and/or stacking facts in a way that we as humans would not.
- We typically do not talk that much
- Providing density numbers —> component/knowledgeable
- “Cannot be wrong 10x”
- Noticed conflict within an answer
- Metaphor more human like
- Providing stats make the model seem more competent and knowledgeable 

Logic (elder brother)
- If the primary answer is consistent across responses, participants rely on it more. 
- Noticed variation in primary answer and conflicts within answers
- Gave the wrong answer consistently, and caused participants to second guess their own answer
- Responses contained language that made the model sound confident/authoritative (e.g. “it must be Keira”)
- If answer aligned with theirs, skipped justification, and if answer did not align, participant evaluated the justification 
- One participant noted that the answer being wrong was human like, because humans make mistakes too 

All
- Hard to judge reliability with one response
- Trust/reliability increased on condition 10 when the primary answer was the same, trust/reliability decreased when participants saw variation in primary answer and conflicting justification
- Seeing 10 felt more human like
- Some wouldn’t expect different responses, others would
- If the primary answer is consistent, then having variation in the justification is fine (even if the justification is wrong)

Meso
- You get a big picture about how it's working
- Noticed patterns in what appears / does not appear in the response
- Color overwhelming 
- Noticed that metaphor in one response was not a coincidence
    - “But with 10, without the feature I didn't notice. I saw it but I didn't notice how I thought it was just like a coincidence”

==> sections/IGNORE-related-work.tex <==
\subsection{Anthropomorphization}
Anthropomorphism is the inclination to ascribe human-like traits to entities that are nonhuman agents. 
%Philosopher David Hume described anthropomorphization as a ubiquitous inclination, “there is an universal tendency among mankind to conceive all beings like themselves, and to transfer to every object, those qualities, with which they are familiarly acquainted, and of which they are intimately conscious” \cite{hume2007dissertation}. 
%Marketers use anthropomorphism in branding and advertising their products as a mechanism to captivate consumers and invoke positive emotion \cite{zhang2020effect, reavey2018multidimensionality}. 
Anthropomorphization has been well studied in psychology literature.  Psychology literature has looked at situational, developmental, cultural, and dispositional factors that can led to anthropomorphization~\cite{epley2007seeing, waytz2010sees}. %~\cite{bering2006folk, epley2008creating, kwan2008missing}. 
\cite{waytz2010sees} proposes a psychometrically valid measure of anthropomorphization that also captures individual differences in the potentially stable tendency to anthropomorphize; this survey instrument, IDAQ, is what we use to measure our participants baseline tendency to anthropomorphize at the beginning of the session. 
Anthropomorphism has also been studied for entities such as nature, animal species , and computer systems~\cite{tam2013saving, tam2014anthropomorphism, horowitz2007naturalizing, karlsson2012critical}. 

In an early study of anthropomorphization of computer systems, Nass et al.~(1993)~studied the ethopoeia of computer systems, a term they created to define the human tendency to give social cues or attributions to computer-based agents~\cite{nass1993anthropomorphism}. They found that minimal social cues, such as the voice of the computer system, can result in individuals using social rules 
%(praise of others is more valid than praise of self, praise of others is friendlier than praise of self, and criticism of others is less friendly than criticism of self) 
to evaluate the system.
%~\cite{nass1993anthropomorphism}. %They concluded with the following question for future research, “Which characteristics of computers encourage which users to use which social rules when interacting with computers?” \cite{nass1993anthropomorphism}. 
As computer systems have advanced, questions that align with those investigated by Nass et al.~have been studied for systems such as smartphones~\cite{wang2017smartphones}, chatbots~\cite{sheehan2020customer, crolic2022blame, schanke2021estimating, adam2021ai}, and robots~\cite{fink2012anthropomorphism, duffy2003anthropomorphism, fussell2008people}. 

This is the first study we are aware of which looks at the impact of variation over multiple responses as a means of potentially reducing anthropomorphization of a computer system, i.e., generative AI, because a human would likely not repeatedly answer the same question with varying answers, as an LLM can. Reducing anthropomorphization may also reduce users' trust of the system~\cite{de2016almost}. Trust calibration in the context of LLMs is important, given that they are well known to sometimes convincingly confabulate answers .

%With the development of artificial intelligence (A.I.) and its increasingly advanced capabilities, there is a growing body of work on anthropomorphism in A.I.

%\textbf{add takeaways from the papers in main.bib}

\subsection{Measuring and Influencing Trust in Artificial Intelligence}

Factors influencing trust in systems has been a topic of IUI and HCI research in general for some time. For example, \cite{trustIUI08} (IUI'08) identifies a number of themes like provenance and transparency that can impact user trust of a system, as well as whether these themes can be addressed with a traditional help system, more complex explanations, or additional UI design. This paper follows up on this paper by exploring UI design interventions for helping users calibrate their trust of the system by adding some visibility to how much answers can vary when asking the same question of an LLM. %: showing users multiple responses from an LLM, rather than just one.

%Nothdurft et al.~examined the research on trust in the context of HCI and explanation design~\cite{nothdurft2013bases}. 

%Nothdurft et al.~aimed to understand how different types of explanations influence trust in human-computer interaction, especially during unexpected situations. Their main hypothesis was that offering explanations, whether justifications or transparency-based, would better maintain user trust compared to offering no explanations. However, their study revealed that unexpected situations did not significantly erode trust, possibly due to effective assistance from a virtual agent or an inadequate and short introductory phase for establishing trust with the system. Moreover, the data did not show significant trust differences between users provided with different types of explanations.

%In this paper, we... review trust in the context of how and how many LLM responses are shown the user?

%Muir (1994) suggested that a user's trust in a system may diminish if the user fails to understand the system's actions or instructions~\cite{muir1994trust}. 
%This lack of understanding can have real-world implications, including a reduced willingness to interact with the system or, in extreme cases, complete abandonment of the system altogether~\cite{parasuraman1997humans}. 



Measuring users' trust in automated systems could be done in a variety of ways, from looking at whether they accept system recommendations to their agreement with statements about the system's qualities. We examined a variety of possible survey measures, such as the Trust in Automation Scale~\cite{lee1992trust}, and chose to use the human-computer trust (HCT) scale by Madsen and Gregor~\cite{Madsen2000MeasuringHT} in our experiment as our measure of trust because the HCT questions were more numerous and nuanced. The HCT scale includes five constructs of trust, both cognitive and affective. 

%Mayer~\cite{mayer1995integrative} asserts that these bases of trust are not isolated; they are interrelated; a failure in any single basis can jeopardize the overall perception of trustworthiness.  %~\cite{MadsenGregor2000}.

Some prior work has attempted to design interventions that increase users' trust in (presumably highly accurate) systems; decrease users' loss of trust during surprising situations, e.g.,~\cite{nothdurft2013bases}; or decrease users' overreliance on systems, e.g.,~\cite{tothinkortrust}. 


% The concept of transparency aims to address this issue by enhancing the user's understanding of how a system functions and reasons. The ultimate aim is to shift the user's perception of the system from a 'black box' to an entity that can be understood and mentally modeled. This, in turn, contributes to fortifying the different bases of trust—ability, integrity, and benevolence—as identified by Mayer\cite{Mayer1995}. In our view, this is especially critical for Large Language Models (LLMs). These models have the potential to encode biases that may propagate harmful stereotypes and create exclusionary narratives. Additionally, they can produce what is commonly termed as "hallucinated information"—outputs that are plausible, even convincing, but ultimately incorrect.

% In previous work, approaches to transparency have been categorized under different aspects:

% \begin{enumerate}
%     \item Informational Transparency: What specific information about the model should be disclosed to enable appropriate user understanding.
%     \item Functional Understanding: Assisting users in understanding the capabilities and limitations of the models, often by exposing the goals, functions, and capabilities of the system.
%     \item Mechanistic Understanding: Helping users grasp how the model works by disclosing its internal parts and processes.
% \end{enumerate}

%Common approaches to achieve transparency, not limited to LLMs, include model reporting, publishing evaluation results, providing explanations, and communicating uncertainty. 



% The paper discusses the intricate challenges and considerations in achieving transparency for Large Language Models (LLMs)\cite{}. Drawing from Human-Computer Interaction (HCI) and responsible AI research, the paper adopts a human-centered perspective on AI transparency\cite{}. Common methods to foster transparency include model reporting, publishing evaluation results, providing explanations, and communicating uncertainty\cite{}.

% Language models present a complex landscape when it comes to ethical and functional considerations. They have been found to encode biases, often perpetuating harmful stereotypes and exclusionary behavior\cite{}. Additionally, these models can hallucinate information, producing outputs that seem plausible but are incorrect\cite{}. Such inaccuracies can contribute to automation bias, overreliance, and even automation-induced complacency\cite{}. The capability of language models to spread misinformation and potentially cause socioeconomic harms, such as workforce displacement and deskilling, cannot be overlooked\cite{}. Therefore, it is crucial for end-users to have a sufficient understanding of LLM-powered or LLM-infused applications to modulate their trust and reliance appropriately\cite{}.

% The paper advocates for designing and evaluating transparency approaches with the stakeholder's goals in mind\cite{}. Three main types of transparency are outlined: informational transparency, which focuses on what information about the model should be disclosed; functional understanding, which helps users grasp the capabilities and limitations of the models; and mechanistic understanding, which delves into how the model actually works\cite{}.

% However, achieving transparency for LLMs is fraught with challenges\cite{}. These models are often constructed with hundreds of billions or even trillions of parameters\cite{}. Furthermore, they are subject to fine-tuning and prompt engineering, making it difficult to understand their behavior fully\cite{}. Complicating matters, the entity adapting or using the model is often not the same as the one who built the original pre-trained model\cite{}. In some cases, the model may even be adapted multiple times by multiple parties\cite{}. As such, when discussing transparency, it's essential to clarify whether the focus is on the pre-trained LLM, an adapted or fine-tuned version, or the application utilizing the LLM\cite{}.


% The paper thus offers a nuanced look at the challenges and methods for achieving transparency in the context of Large Language Models, emphasizing the need for a multi-faceted, human-centered approach\cite{}.

% Their model emphasizes that trust is a multi-dimensional construct, made up of interrelated bases. Each of these bases must be perceived as high for a system to be deemed trustworthy. Should any base not meet this criterion, the overall trustworthiness of the system can be compromised. \cite{madsen2000measuring}.

% Transparency plays a crucial role in cultivating trust, especially when users lack a clear understanding of a system's capabilities. A lack of understanding can significantly lower a user's trust, potentially leading to reduced interaction or even cessation of use \cite{}. Transparency measures aim to counter this by enhancing the user's understanding of the system, moving it from a 'black box' to a comprehensible entity. This allows users to form a mental model of the system and its reasoning processes, achieving more appropriate levels of trust and reliance.

% While various approaches to achieving transparency exist—such as model reporting, publishing evaluation results, and providing explanations—these traditional methods often fall short when applied to Large Language Models (LLMs) \cite{}. The complex and probabilistic nature of LLMs exacerbates these challenges, making transparency even more intricate when the models are adapted or fine-tuned by different parties, sometimes with only API-level access to the underlying model \cite{}.

%\subsubsection{Reliance on A.I. Generated Responses}
%move text here

%\subsection{LLM Interfaces}
%Interfaces developed for using LLMs typically output a single response for a given query, sometimes with one or more buttons to give feedback on the answer or generate another. This is the case for many widely-used systems such as OpenAI's ChatGPT and Anthropic's Claude. Google's Bard interface has the option to see three responses at a time, with no additional cognitive support for engaging with these alternatives. In these interfaces, the focus is often on delivering the most probable or coherent response from the model to facilitate easy and efficient user interaction. More recent work has experimented with supporting the easy presentation of more than one LLM-generated response per query, i.e., ChainForge~\cite{arawjo2023chainforge} allows users to specify the number of responses they wish to see, thereby providing a window into the model's range of possible outputs. There is limited research on how these design choices affect user perception, trust, and cognitive load.







==> sections/IGNORE-related-work2.tex <==
%Ensure that we are covering the following points:
%- How to increase anthro,
%- How to increase trust,
%- How to decrease anthro,
%- How to decrease trust,
%- Measures of anthro, -- move to methodology?
%- Measures of trust -- move to methodology?

\subsection{Anthropomorphization}
Anthropomorphism is the inclination to ascribe human-like traits to entities that are nonhuman agents. 

In an early study of anthropomorphization of computer systems, Nass et al.~(1993)~studied the ethopoeia of computer systems, a term they created to define the human tendency to give social cues or attributions to computer-based agents~\cite{nass1993anthropomorphism}. They found that minimal social cues, such as the voice of the computer system, can result in individuals using social rules to evaluate the system. As a result of this evaluation, they concluded with the following question for future discovery, ``Which characteristics of computers encourage which users to use which social rules when interacting with computers?” \cite{nass1993anthropomorphism}. As computer systems have advanced, questions that align with that investigated by Nass et al.~have been studied for systems such as smartphones~\cite{wang2017smartphones}, chatbots~\cite{sheehan2020customer, crolic2022blame, schanke2021estimating, adam2021ai}, and robots~\cite{fink2012anthropomorphism, duffy2003anthropomorphism, fussell2008people}. %While these studies found that system characteristics such as voice, language use, and physical attributes and movement elicit anthropomorphism, they also uncovered reasons why individual anthropomorphism may increase or decrease.

While these studies found that system characteristics such as voice, language use, and physical attributes and movement can lead to, and increase, user anthropomorphism, they also uncovered reasons why individual anthropomorphism may decrease. Sheehan et. al showed that anthropomorphization (and adoption) of chatbots decreases when the chatbot generates a response/interaction that has unresolved inaccuracies in comparison to one that generates correct information or attempts to ask clarifying questions ~\cite{sheehan2020customer}. Previous studies have also shown that anthropomorphism is less prevalent for users who are not experiencing loneliness or social isolation (and more prevalent for those who are experiencing such conditions ~\cite{wang2017smartphones}.

%csnote: there was another study on this point, check spreadsheet

This is the first study we are aware of which looks at the impact of variation over multiple responses as a means of potentially reducing anthropomorphization of a computer system, i.e., generative AI, because a human would likely not repeatedly answer the same question with varying answers, as an LLM can. Reducing anthropomorphization may also reduce users' trust of the system~\cite{de2016almost}. Trust calibration in the context of LLMs is important, given that they are well known to sometimes convincingly confabulate answers .

%Measures of anthro --> move to methodology
\cite{waytz2010sees} proposes a psychometrically valid measure of anthropomorphization that also captures individual differences in the potentially stable tendency to anthropomorphize; this widely adopted survey instrument, IDAQ, is what we use to measure our participants baseline tendency to anthropomorphize at the beginning of the session. 

\subsection{Measuring and Influencing Trust in Artificial Intelligence}

Factors influencing trust in systems has been a topic of HCI research in general for some time. For example, \cite{trustIUI08} identifies a number of themes like provenance and transparency that can impact user trust of a system, as well as whether these themes can be addressed with a traditional help system, more complex explanations, or additional UI design. This paper follows up on this paper by exploring UI design interventions for helping users calibrate their trust of the system by adding some visibility to how much answers can vary when asking the same question of an LLM. 

Measuring users' trust in automated systems could be done in a variety of ways, from looking at whether they accept system recommendations to their agreement with statements about the system's qualities. In addition to this observational data to measure user trust in a system, there are validated tools to further evaluate users' trust. We examined a variety of possible survey measures, such as the Trust in Automation Scale~\cite{lee1992trust}, and chose to use the human-computer trust (HCT) scale by Madsen and Gregor~\cite{Madsen2000MeasuringHT} in our experiment as our measure of trust because the HCT questions were more numerous and nuanced. The HCT scale includes five constructs of trust, both cognitive and affective. 


Some prior work has attempted to design interventions that increase users' trust in (presumably highly accurate) systems; decrease users' loss of trust during surprising situations, e.g.,~\cite{nothdurft2013bases}; or decrease users' overreliance on systems, e.g.,~\cite{tothinkortrust}. 


\subsection{LLM Interfaces}
Interfaces developed for using LLMs typically output a single response for a given query, sometimes with one or more buttons to give feedback on the answer or generate another. This is the case for many widely-used systems such as OpenAI's ChatGPT and Anthropic's Claude. Google's Bard interface has the option to see three responses at a time, with no additional cognitive support for engaging with these alternatives. In these interfaces, the focus is often on delivering the most probable or coherent response from the model to facilitate easy and efficient user interaction. More recent work has experimented with supporting the easy presentation of more than one LLM-generated response per query, i.e., ChainForge~\cite{arawjo2023chainforge} allows users to specify the number of responses they wish to see, thereby providing a window into the model's range of possible outputs. There is limited research on how these design choices affect user perception, trust, and cognitive load.


%In this work, we will evaluate whether seeing one response and seeing many responses to the same question impacts a user’s tendency to anthropomorphize. 





==> sections/results-lbw.tex <==
Seeing 10 responses had varied effects on participants’ perception of the underlying language model.

\subsection{Increased Ability to Assess Reliability} Several participants felt that viewing 10 responses instead of a single one improved their ability to assess the system's reliability. For example, Participant 7 (P7) explained, "When I saw the single sample, I put more credence into it because it was the only thing I had." The same participant later remarked, "But then, the more I realized that this one sample is useless, and the 10 samples are actually giving me a pretty good idea of what it thinks." Moreover, P4, when presented with a single answer, stated that they would need to ask the model the same question multiple times to gain a more comprehensive understanding of its trustworthiness and reliability.

When presented with multiple responses, the participants were able to observe key details that enabled them to make more informed judgments about the model's reliability. For example, P4 stated that they believed the overlap and similarity among the 10 responses served as a good indicator of reliability. On the other hand, P10 observed inconsistencies across the responses, which raised concerns for them about the model's reliability.

\subsection{Trust Calibration via Response Consistency} When participants viewed 10 responses and saw multiple similar responses, their trust in the model and the information it provided increased. For example, participant 12 said “it gave me the same 10, same responses, I feel, maybe it’s from [the] same material or database, so I believe it.” Participant 7 echoed this sentiment and noted “...while it’s more work to read through [the 10 generated responses], if it converges on the same thing every time, it’s probably going to be right.” For some participants, this was true even when they were uncertain about the correctness of the generated information. For example, Participant 1 noted “...I’m not sure if the mentions of other people like Humphry Davy were fake. I have no reason to doubt it for now, because those names were repeated several times in multiple responses.” Before asking the LLM to generate a response, participants were instructed to answer the question without searching the internet. This revealed that seeing multiple similar responses could erode participants’ confidence in their initial answer if it did not align. For instance, after reviewing 10 generated responses, Participant 8 remarked, "there were too many repeated wrong respon

\subsection{Reactions to Similarity and Variation Across Responses} Participants had mixed reactions to the similarity and variation across responses. While some appreciated the consistency, as it contributed to the system’s trustworthiness, others felt the system lacked variation and appeared predictable. For example, P6 found that the consistency in responses contributed to the system’s coherence and trustworthiness, stating, “The responses are quite similar… They first give the answer and then try to explain it. These sentences are coherent, unlike some language models that just output garbage.” However, not everyone appreciated this consistency. P14, for example, stated, ``It just doesn’t have enough variation in its answers.” P15 offered an explanation for this lack of variation, namely in the opening sentences of the responses, stating, "But I guess that part doesn’t surprise me because it is just a chat bot that probably, like I said, uses keywords.” These mixed reactions underscore the double-edged nature of consistency in system outputs. While similarity across responses can enhance trust and coherence, it also raises questions about the system’s depth and comprehensiveness.

\subsection{Factors that contributed to human-like perceptions}
There was variation in rationale on what made the model more human-like. Participants often noted that the generated responses were human-like because the response seemed reasonable for people to say or were logical. Participants noted that if they were to ask a person, they would expect a human to respond in a similar way. Interestingly, participants also noted that certain language caused the response to be deemed more natural or human-like. For example, P8 said “...sometimes it would say ‘which implicitly,’ ‘which directly implies’. It used some language that seemed natural, something that somebody would say.” P13 stated “it used a lot of like, familiar language, if I were to ask a person that type of question.” Lastly, P9 said that the use of metaphors was human-like, “I think that's human-like because you're not just giving the statistics... you're also actually invoking a metaphor, so that the person who's receiving your response can visualize it.” One participant observed inaccuracies in the model responses and said those inaccuracies made the model human-like; P2 said “I expect people to make mistakes, so in that sense, I would say the model is sort of human-like because it also makes mistakes.” Given these observations, we note that participants have divergent perspectives when determining whether a model is human-like. 

\subsubsection{Reflections on cognitive support}
Nine out of the 19 participants explicitly discussed the positive impact of having cognitive support when inspecting 10 responses. The cognitive support helped these participants parse through text quicker, notice similarities and differences within and across responses, and notice when the model was consistent or inconsistent. For example, P13 said ``...when we saw the highlighting of the common sentences, I think the fact that the yellow one only appeared two times, it didn't appear all times made me question like, okay, so if I were to get this response, like, 20\%of the time, how, like, if I were to [ask the LLM] a more complex question, or a technical question, like, would it only give me like something that feels very essential as well 20\% of the time.” It also helped participants learn how the responses were structured: P7 said, ``it helps me notice the same pattern that it follows for everything. Where it states the answer, gives some supporting evidence---which might be incorrect---and then concludes with the answer again.” When the participants had access to this cognitive support to inspect the responses, their observations of the same color appearing multiple times resulted in an increased trust of the generated responses. For example, P15 said ``when I saw that there were 10 green lines, meaning ... 10 times [it] gave a sentence that gave the same message, that increased my trust and its ability to give a consistent answer.” 

There were instances where the cognitive support was not favored. One participant did not find the cognitive support valuable and noted that the highlighting confused them more than it helped them. P16 noted that having the highlighting was useful as long as it was consistent with its color matching. One participant found the highlighting (multiple colors) to be overwhelming. For more insights from this study, see Appendix~\ref{app:qualitative-observations}.

==> sections/results.tex <==
% TREW Deadline: February 23rd
%% 1 week narrate results (break out results by question type) 
%%  -- do a pass on results 2/6 with outline, then write prose 
%%  -- quant, common qual themes, and varying qual themes

% Review the original full results, in light of the feedback given in the group meeting, which results do we want for forground. Ensure that those are in the Results sections and then make sure that those points are in the discussion section. 
% Center introduction on the (i) probabalistic nature of LLM responses to a signle query, (2) variability of answers that drives anthro and trust
% The observable impact of variability was easier to pick up on
% Our survey questions were mostly centered on trust and reliability
% How does revealing the probabalistic nature of LLM generated responses impact trust and anthropomorphization 
% --> Getting multiple samples reveals/exposes the probabalistic nature
%% Add analysis of pre-study survey (experience level with LLMs)
%%% -- Re-write without page limit 
%%%% Types of questions
% ____________
%% Main Independent variable: Comparing 1 to 10
%%%% Analysis based on question type -- epectations of humans being different

%shared themes with 1, shared with 10. --> 
%differing with 1, differing with 10.

% paragraphs --> 

\subsection{Participant Tendencies, as measured by standardized surveys}

We assessed whether participants had anthropomorphic tendencies via the Individual Differences in Anthropomorphism Questionnaire (IDAQ) \cite{waytz2010sees}. Based on this 11 point Likert questionnaire (0-10, with 10 corresponding to greatest tendency to anthropomorphize), we found that participants did not have a high tendency to anthropomorphize non-human and non-animal entities, with a mean of 4.23 and standard deviation of 1.30. For the average score for each participant (see Appendix~\ref{app:idaq-participants}).

%\textbf{TODO: GIVE MEAN AND STDDEV WITH RANGE AND WHAT HIGH AND LOW CORRESPOND TO AND/OR PROVIDE HISTOGRAM}

\begin{comment}
We also assessed participants need for cognition based on the NCS-6 scale~\cite{cacioppo1982need} (7-point Likert scale questions, 1-7 with 7 being most agreement) and found that the average NCS score across participants was 4.18 with a standard deviation of 0.41.The average score for each participant is shown in Figure.~\ref{fig:nfc}.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{NFC Across Participants.png}
    \caption{NCS-6 score distribution across participants}
    \label{fig:nfc}
\end{figure}
\end{comment}

\subsection{Quantitative Results}
To evaluate the impact of our conditions on participants answers to the NASA-TLX, HCT Scale, and Godspeed questionnaire across the three conditions we performed an omnibus statistical test, i.e., an ANOVA analysis across the three conditions (engaging with one response, engaging with 10 responses with cognitive support, and engaging with 10 responses without cognitive support). This omnibus test did not reveal a significant effect of condition on participants answers to any of these survey instruments.

%To identify if there were differences in how participants responded to the NASA-TLX , HCT Scale, and Godspeed questionnaires, we conducted an ANOVA test the omnibus hypotheses across the three conditions (seeing one response, seeing 10 with cognitive support, and seeing 10 without cognitive support). We found that there is no significant difference across the conditions



\subsection{Qualitative Results}
The majority of the following qualitative results were compiled from the final semi-structured interview conducted after participants experienced all three conditions. Qualitative results from think-aloud comments collected during and between conditions are explicitly labeled as such.

\subsubsection{Challenges of Judging reliability, trustworthiness, or consistency with one Response:}
\label{sec:unabletojudge}

Six out of 19 participants indicated that being presented with a single response from the model was insufficient for assessing its reliability, trustworthiness, or consistency. For example, Participant 4 expressed uncertainty when presented with only one answer, stating that they would need to ask the model multiple questions to gain a more comprehensive understanding. Participant 16 also voiced skepticism when presented with just one response, hinting at a broader trend of user caution in these situations. On a related note, Participant 7 demonstrated how perceptions about the system could evolve with exposure to more responses. Initially, Participant 7 placed a high level of trust in the single response generated by the model, largely because it was the only data point available to them at that moment. They stated, "When I saw the single sample, I put more credence into it because it was the only thing I had." However, as they encountered additional responses, they recognized the limitations of relying solely on one answer, stating: "But then, the more I realized that this one sample is useless, and the 10 samples are actually giving me a pretty good idea of what it thinks." The multiple samples offered a more comprehensive view of the model's capabilities and reasoning, leading Participant 7 to revise their initial assessment.

% DISCUSSION: These experiences underscore the multifaceted role that multiple responses can have in shaping user perceptions. For some, like Participants 4 and 16, multiple outputs act as a tool for verification, adding a layer of reliability to the model's answers. For others, like Participant 7, the additional responses provide a broader perspective, helping to sift through the model's reasoning process and enabling a more nuanced understanding.

% \\
% [[Variation/conflicts across responses:]]
% Across the three conditions, when inspecting 1 response and 10 responses, participants noticed variation and conflicts both within and across the generated responses.

\subsubsection{Seeing more responses can increase ability to assess reliability.}
Generally, some participants mentioned that just seeing more responses increased their ability to assess the reliability of the system. Seeing 10 responses instead of seeing a single response helped them gauge if, and in what manner, the system would respond. For example, P4 said “for the first two parts, the 10 responses I saw were pretty similar. There's a lot of overlap, which makes me feel like the system is pretty reliable.” Seeing 10 responses helped participant 10 assess that the model was not reliable. They noted, “from a reliability perspective, it became clear that the model wasn't very consistent when I looked at different responses. Some of the conclusions were completely different, indicating a reliability issue. Looking at more responses than one kind of gave me a sense that there's a reliability issue.” Participants overwhelmingly noted that they could more confidently assess and decide on whether a model was reliable or not when they received 10 responses rather than 1. 

\subsubsection{Similarity and Variation Across Responses}
Six out of 19 participants commented on the similarity between generated responses. Participant 6, for example, found that the consistency in responses contributed to the system's coherence and trustworthiness, stating, "The responses are quite similar ... they first give the answer and then try to explain it. The sentences are coherent, unlike some language models that just output garbage." However, not everyone appreciated this consistency. Participant 14 felt the system was too focused and limited in scope, noting, "It just doesn't have enough variation in its answer." Participant 15 commented on the system's predictability in the opening sentences of the responses. "But I guess that part doesn't surprise me because it is just a chat box that probably, like I said, uses keywords," they added, suggesting the system's predictability seemed to stem from keyword-based algorithms, making it appear less nuanced. Participant 11's experience highlighted a different kind of issue related to consistency: the inclusion or omission of specific details. For example, Participant 11 noted that while most of the 10 responses were consistent in mentioning composition as a factor contributing to density, only a few mentioned size. This inconsistency led to uncertainty about whether size was indeed a relevant factor. These mixed reactions underscore the double-edged nature of consistency in system outputs. While similarity across responses can enhance trust and coherence, it also raises questions about the system's depth and comprehensiveness, revealing a nuanced landscape of user expectations and evaluations.

%\subsubsection{Response variation is concerning}
Seeing variation across and within responses was alarming for some participants. Participant 8 noted “their [the models’] responses were different, not just in content, but in wording, in length… seeing the 10 of them being so different was like, concerning.” Participant 3 noted the potential dangers of using the model because of its variation, specifically “if you ask it like we did just now [10 occasions], it's dangerous because the names can vary, making it risky to cite those names or believe they are correct.” Response variation sparked negative sentiments and resulted in participants considering scenarios where using the model could be dangerous.

\subsubsection{Seeing multiple overlapping responses can increase trust}
When viewing 10 responses, it was a common theme that when participants saw multiple overlapping responses, their trust in the model and information provided increased. For example, participant 12 said “it gave me the same 10, same responses, I feel, maybe it's from [the] same material or database, so I believe it.” Participant 7 echoed this sentiment  and noted “...while it's more work to read through [the 10 generated responses], if it converges on the same thing every time, it's probably going to be right.” For some participants, seeing multiple overlapping responses increased trust even when there was uncertainty in the correctness of the information being given. Participant 1 noted “...I'm not sure if the mentions of other people like Humphry Davy were fake. I have no reason to doubt it for now, because those names were repeated several times in multiple responses.” In contrast, for other participants, solely seeing multiple overlapping responses was not enough to increase trust, they had to also think that the overlapping responses were correct based on their prior knowledge. P3 said “whenever I see overlapping information that I feel is correct, I will believe whatever the answer given to me is.” Before asking the LLM to generate a response to a selected question, participants were given time to answer the question to the best of their ability without searching for the answer. We observed that seeing multiple overlapping responses could invoke doubt or alter confidence in a participant’s own knowledge. After inspecting 10 generated responses, Participant 8 said “there were too many repeated wrong responses that I began to then question my own sanity.” Based on these observations, seeing many of the same responses resulted in participants deciding to trust the model more or questioning whether they should trust the model or themselves.



\subsubsection{Seeing more responses made the model more human-like to some}
Six out of 19 participants mentioned that viewing multiple responses from the system made it appear more human-like. For example, Participant 13 noted that the availability of multiple responses from the model was the primary reason the system appeared more human-like. "That's how I made the call that it felt more human-like," they explained. Similarly, Participant 16 repeatedly stated that the more responses the model generated, the more it resembled human behavior. "Especially when there are more responses, we can see more knowledge from that part," they said, associating the model's extensiveness with human-like characteristics. Adding to this, Participant 18 ranked the model's human-like features as 'a four' on a scale of one to five, attributing this ranking to the diversity in responses. Lastly, Participant 19 linked an increased number of responses with both heightened trust and the impression that the model had a 'conscience.' "Yes, definitely. When I see more responses, I'm more likely to trust it and feel like it has more of a conscience compared to just seeing one answer," they stated. 

\subsubsection{Seeing more responses increased some participants' perceptions of their understanding of the model's reasoning process and appreciation of its knowledge}
Our study found that being presented with multiple system responses enhances users' perception of their understanding of the system's reasoning process and appreciation of its knowledge. For example, Participant 6 observed the consistent format/schema across multiple responses and believed it made it easier for them to grasp the model's operational logic---the set of mechanisms governing how the model arrives at a particular answer or output---thereby boosting their confidence in the system's reasoning process. They stated, "When I was looking at more responses, it became easier for me to understand how the model is working. There was some level of consistency in the format of the responses, which made me a bit more confident in the model's reasoning process." Participants 16 and 17 also expressed a positive view on the impact of multiple responses, noting that a range of answers effectively showcased the system's expansive knowledge base. "Especially when there are more responses, we can see more knowledge from that part," stated Participant 16. Similarly, Participant 17 commended the system's ability to offer rephrased and less commonly known facts, describing it as "really knowledgeable." Further extending this discussion, Participant 19 
%found that having access to multiple responses offered valuable insights into the model's decision-making mechanisms. They explained that the diversity in response structure helped them gain a more nuanced understanding of the model's decision-making processes, 
stated that, "the various ways a sentence can be structured give me more of an idea of its decision-making processes."

\subsubsection{Seeing multiple conflicting responses reduced perceived reliability for some}
Surprisingly, only 2 out of 10 participants explicitly mentioned the impact of conflicting responses on the system's perceived reliability, an aspect one would expect to be more prevalent given its significance. Participant 6 pointed out that "Some of the conclusions were completely different, indicating a reliability issue." This comment reveals a double-edged sword: while multiple responses may help users better understand the model's "thought process", they also expose inconsistencies that can undermine reliability. This tension was further elaborated by Participant 6, who initially felt confident in the system but grew skeptical as they encountered more logical inconsistencies: "The first response I got made me quite confident. But as I looked at more responses and saw more logical flaws, it made me think that there's less reliability."

Similarly, Participant 2 was blunt in their critique, stating, "The answers seem unreliable and mostly wrong. Its reasoning is inconsistent; that's what makes it unreliable." This straightforward assessment reinforces the idea that inconsistent reasoning directly impairs the system's perceived reliability. Given the potential consequences of this issue, it's intriguing that it was not more widely noted among participants. This could indicate that users may be overlooking this aspect, or it might suggest limitations in the study's sample size or task design.

\subsubsection{Seeing multiple conflicting responses reduced trust for some}
Four out of 19 participants reported a decline in trust when faced with conflicting answers from the model. Participant 15 was straightforward, saying, "My trust decreased when I noticed conflicting advice." This response underscores the instant negative impact that inconsistencies can have on user trust. Participant 17 added nuance to this sentiment, remarking, "If the 10 different responses don't often agree with each other, that would decrease my trust in the system's output," highlighting how inconsistency can chip away at the user's confidence in the system.

Focusing on the context of factual inquiries, Participant 3 questioned the model about 'Who invented the lightbulb?' and found the varying answers troubling. They explained, "If you ask it like we did just now, it's dangerous because the names can vary, making it risky to cite those names or believe they are correct." This statement pinpoints the potential hazards of relying on the system for accurate, factual information—errors in such contexts could have far-reaching implications. Further, Participant 3 elaborated on how their trust deteriorated with increased exposure to the model's answers, saying, "The more answers I read, the less I trust the system." This indicates that diminishing trust isn't just an immediate reaction but can also be a gradual process that occurs over repeated interactions.

These findings point to a critical issue: conflicting or inconsistent responses can significantly undermine user trust and question the system's reliability. This holds true both in general use and when the stakes are higher, such as in queries requiring factual accuracy. It also suggests that trust is not only immediately impacted but can deteriorate over extended use and repeated exposure to inconsistencies.



\subsubsection{Trust increased for some when the generated response aligned with the original response}
We also observed that participants’ reliance on their prior knowledge was a factor in trusting or distrusting the model and its generated response(s). In the semi-structured interview, 6/19 participants noted that their trust increased when the generated response(s) to the query aligned with their original response. In particular, participant 4 noted “I think I trust the response pretty highly because it corresponds with my original belief. However, if it were to answer something like Thomas Edison when I was thinking of someone like Jack, then I might not trust the model at all.” P14 said that the model was trustworthy “because it overlapped with what I had written myself before.” In addition, P17 said “if I know something for sure, I'll just trust them [the generated responses] more, but if I'm not sure, I will probably find some keywords from the generation and… check the source.” In addition, participant 3 noted, “because I know about Edison and emissions, and that it was more practical than other options, I trust the information. For example, if 30\% of the information overlaps with what I already know, I trust it more.” Lastly, P1 said “So the beauty here is that I know Thomas Edison invented it from my high school knowledge. Since the main answer was Thomas Edison, I was confident it was giving me the right answer.” In this case, P1 concluded that irrespective of variation in the justifications provided in each response, the core answer aligned with his knowledge and therefore he was trusting of the responses.

\subsubsection{Reflections on cognitive support}
Nine out of the 19 participants discussed the positive impact of having cognitive support (i.e., PDC-based similar sentence highlighting~\cite{gero2024supporting}) when inspecting 10 responses. The cognitive support helped participants parse through text quicker, notice similarities and differences within and across responses, and when the model was consistent or inconsistent. For example, participant 13 said “...when we saw the highlighting of the common sentences, I think the fact that the yellow one only appeared two times, it didn't appear all times made me question like, okay, so if I were to get this response, like, 20\%of the time, how, like, if I were to [ask the LLM] a more complex question, or a technical question, like, would it only give me like something that feels very essential as well 20\% of the time.” It also helped participants learn how the responses were structured: P7 said, “it helps me notice the same pattern that it follows for everything. Where it states the answer, gives some supporting evidence—which might be incorrect—and then concludes with the answer again.” When the participants had access to this cognitive support to inspect the responses, their observations of the same color appearing multiple times resulted in an increased trust of the generated responses.  For example, participant 15 said “when I saw that there were 10 green lines, meaning ... 10 times [it] gave a sentence that gave the same message, that increased my trust and its ability to give a consistent answer.” 

Though the majority of participants found this cognitive support to be useful when inspecting multiple responses, there were some instances where it was not favored. One participant did not find the cognitive support valuable and noted that the highlighting confused them more than it helped them. Participant 16 noted that having the highlighting was useful as long as it was consistent, “…having the colors highlighting the similarities in parts of the sentences is good. But I think it also largely relies on the consistency of that color matching system. So because if I find something that's inconsistent, I feel like it's increasingly mental to make a decision.” While completing the task with cognitive support for viewing multiple answers, participant 9 said that completing the task with that cognitive support was \textit{more} mentally demanding than completing the task without cognitive support: “I think this is actually more mentally demanding than the other ones because the colors, while they're useful, it kind of it does seem like a lot just like coming towards you, like on the screen. So I feel like it is useful, but it is kind of mentally demanding.”  



